Search for the $b\bar{b}$ decay of the Standard Model Higgs boson in associated $(W/Z)H$ production with the ATLAS detector

A search for the $b\bar{b}$ decay of the Standard Model Higgs boson is performed with the ATLAS experiment using the full dataset recorded at the LHC in Run 1. The integrated luminosities used from $pp$ collisions at $\sqrt{s}=7$ and 8 TeV are 4.7 and 20.3 fb$^{-1}$, respectively. The processes considered are associated $(W/Z)H$ production, where $W\to e\nu/\mu\nu$, $Z\to ee/\mu\mu$ and $Z\to\nu\nu$. The observed (expected) deviation from the background-only hypothesis corresponds to a significance of 1.4 (2.6) standard deviations and the ratio of the measured signal yield to the Standard Model expectation is found to be $\mu = 0.52 \pm 0.32 \mathrm{(stat.)} \pm 0.24 \mathrm{(syst.)}$ for a Higgs boson mass of 125.36 GeV. The analysis procedure is validated by a measurement of the yield of $(W/Z)Z$ production with $Z\to b\bar{b}$ in the same final states as for the Higgs boson search, from which the ratio of the observed signal yield to the Standard Model expectation is found to be $0.74 \pm 0.09 \mathrm{(stat.)} \pm 0.14 \mathrm{(syst.)}$.

==> App_MassResolution.tex <==
\begin{figure}[tb!]
\begin{center}
\centerline{
\subfigure[]{\includegraphics[width=0.49\textwidth]{Figures/Appendix/MassResolution/qqZllH125_8TeV_MVASel_2L_2J_2T_LLMMTT_vptIncl_JetCorrSet1_mjj.pdf}}
\subfigure[]{\includegraphics[width=0.49\textwidth]{Figures/Appendix/MassResolution/qqZllH125_8TeV_MVASel_2L_2J_2T_LLMMTT_vptIncl_JetCorrSet2_mjj.pdf}}}
\end{center}
\caption{Dijet-invariant-mass distribution for the decay products of a
  Higgs boson with $m_H = 125$~GeV in the 2-lepton MVA selection. 
The distributions are shown 
(a) using jets after global sequential calibration (GSC, solid), 
and after adding muons inside jets (dotted) 
and after correcting for resolution effects specific to the kinematics of
the decay of a Higgs boson with $m_H = 125$~GeV (dash-dotted); 
(b) using jets after global sequential calibration (GSC, solid), 
and after adding muons inside jets and applying the kinematic fit (dash-dotted). 
The distributions are fit to the Bukin function~\cite{Bukin} and the parameter representing 
the width of the core of the distribution is shown in the figures, 
as well as the relative improvement in the resolution with respect to jets after the global sequential calibration.
}
\label{fig:mass_resolution}
\end{figure}


==> App_Plots_BDTAllRegions.tex <==

% for the moment: keep the format as in the supporting note, showing all inputs to fit
% (which means showing mbb distributions for 0-lepton for ptV < 120)


\begin{figure}[tb!]
\begin{center}
\centerline{
\subfigure[$\ptv<120~\GeV$, 2 jets, 1-tag]{\includegraphics[width=0.30\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA0_B1_J2_T1_L0_distMV1cBTag_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv>120~\GeV$, 2 jets, 1-tag]{\includegraphics[width=0.30\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B2_J2_T1_L0_distMV1cBTag_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv>120~\GeV$, 3 jets, 1-tag]{\includegraphics[width=0.30\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B2_J3_T1_L0_distMV1cBTag_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv<120~\GeV$, 2 jets, LL]{\includegraphics[width=0.30\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA0_B1_J2_T2_L0_distmjj_TTypell_GlobalFit_unconditionnal_mu1.pdf}}
}
\centerline{
\subfigure[$\ptv>120~\GeV$, 2 jets, LL]{\includegraphics[width=0.30\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B2_J2_T2_L0_distmva_TTypell_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv>120~\GeV$, 3 jets, LL]{\includegraphics[width=0.30\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B2_J3_T2_L0_distmva_TTypell_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv<120~\GeV$, 2 jets, MM]{\includegraphics[width=0.30\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA0_B1_J2_T2_L0_distmjj_TTypemm_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv<120~\GeV$, 2 jets, TT]{\includegraphics[width=0.30\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA0_B1_J2_T2_L0_distmjj_TTypett_GlobalFit_unconditionnal_mu1.pdf}}
}
\centerline{
\hfill
\subfigure[$\ptv>120~\GeV$, 2 jets, MM+TT]{\includegraphics[width=0.30\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B2_J2_T2_L0_distmva_TTypexx_GlobalFit_unconditionnal_mu1log.pdf}}
\hfill
\subfigure[$\ptv>120~\GeV$, 3 jets, MM+TT]{\includegraphics[width=0.30\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B2_J3_T2_L0_distmva_TTypexx_GlobalFit_unconditionnal_mu1log.pdf}}
\hfill
}
\end{center}
\caption{
Distributions input to the global MVA fit in the 0-lepton channel:
(a)--(c) MV1c-algorithm output distributions in the 1-tag control regions;
(d), (g), (h) \mbb\ and
(e), (f), (i), (j) BDT$_{VH}$-discriminant distributions in the 2-tag signal regions.
Shown are the data (points with error bars) and expectation (histograms).
The analysis regions ($\ptv$ range, jet multiplicity and $b$-tag region)
are indicated in the subfigure captions.
The bin left boundaries in (a)--(c) denote 
the operating points ({\it{MV1c(b) OP}}) as defined in section~\ref{sec:reco},
corresponding to 
$b$-tagging efficiencies of 80\%, 70\%, 60\%, 50\%,
i.e., the $b$-jet purity increases from left to right.      
The background contributions after the global fit are shown 
as filled histograms.
The Higgs boson signal ($\mh = 125$~GeV) is shown as a filled histogram on top of 
the fitted backgrounds, %both after the global fit (indicated as ``best fit") and 
as expected from the SM (indicated as $\mu=1.0$),
and, unstacked as an unfilled histogram, scaled by the factor indicated in the legend. 
The dashed histogram shows the total background as expected from the pre-fit 
MC simulation. The entries in overflow are included in the last bin.
The size of the combined statistical and systematic uncertainty on the
sum of the signal and fitted background is indicated by the hatched band. The ratio
of the data to the sum of the signal and fitted background is shown in the lower panel.
\label{fig:App_BDTdistributions_0lepton}}
\end{figure}





\begin{figure}[tb!]
\begin{center}
\centerline{
\subfigure[$\ptv<120~\GeV$, 2 jets, 1-tag]{\includegraphics[width=0.2\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B0_J2_T1_L1_distMV1cBTag_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv>120~\GeV$, 2 jets, 1-tag]{\includegraphics[width=0.2\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B0_J3_T1_L1_distMV1cBTag_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv<120~\GeV$, 3 jets, 1-tag]{\includegraphics[width=0.2\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B2_J2_T1_L1_distMV1cBTag_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv>120~\GeV$, 3 jets, 1-tag]{\includegraphics[width=0.2\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B2_J3_T1_L1_distMV1cBTag_TType_GlobalFit_unconditionnal_mu1.pdf}}
}
%
\centerline{
\subfigure[$\ptv<120~\GeV$, 2 jets,  LL]{\includegraphics[width=0.2\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B0_J2_T2_L1_distmva_TTypell_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv>120~\GeV$, 2 jets, LL]{\includegraphics[width=0.2\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B2_J2_T2_L1_distmva_TTypell_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv<120~\GeV$, 3 jets, LL]{\includegraphics[width=0.2\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B0_J3_T2_L1_distmva_TTypell_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv>120~\GeV$, 3 jets, LL]{\includegraphics[width=0.2\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B2_J3_T2_L1_distmva_TTypell_GlobalFit_unconditionnal_mu1.pdf}}
}
%
\centerline{
\subfigure[$\ptv<120~\GeV$ 2 jets, MM]{\includegraphics[width=0.2\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B0_J2_T2_L1_distmva_TTypemm_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv>120~\GeV$ 2 jets, MM]{\includegraphics[width=0.2\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B2_J2_T2_L1_distmva_TTypemm_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv<120~\GeV$, 3 jets, MM]{\includegraphics[width=0.2\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B0_J3_T2_L1_distmva_TTypemm_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv>120~\GeV$, 3 jets, MM]{\includegraphics[width=0.2\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B2_J3_T2_L1_distmva_TTypemm_GlobalFit_unconditionnal_mu1.pdf}}
}
%
\centerline{
\subfigure[$\ptv<120~\GeV$ 2 jets, TT]{\includegraphics[width=0.2\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B0_J2_T2_L1_distmva_TTypett_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv>120~\GeV$ 2 jets, TT]{\includegraphics[width=0.2\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B2_J2_T2_L1_distmva_TTypett_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv<120~\GeV$, 3 jets, TT]{\includegraphics[width=0.2\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B0_J3_T2_L1_distmva_TTypett_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv>120~\GeV$, 3 jets, TT]{\includegraphics[width=0.2\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B2_J3_T2_L1_distmva_TTypett_GlobalFit_unconditionnal_mu1.pdf}}
}
\end{center}
\caption{
The distributions input to the global MVA fit in the 1-lepton channel:
(a)--(d) MV1c-algorithm output distributions in the 1-tag control regions 
and
(e)--(p) BDT$_{VH}$-discriminant distributions in the 2-tag signal regions.
Shown are the data (points with error bars) and expectation (histograms).
The analysis regions (in terms of $\ptv$ range, jet multiplicity and $b$-tag region)
are indicated in the subfigure captions. 
The bin left boundaries in (a)--(d) denote 
the operating points ({\it{MV1c(b) OP}}) as defined in section~\ref{sec:reco},
corresponding to 
$b$-tagging efficiencies of 80\%, 70\%, 60\%, 50\%,
i.e., the $b$-jet purity increases from left to right.      
The background contributions after the global fit of the MVA are shown 
as filled histograms.
The Higgs boson signal ($\mh = 125$~GeV) is shown as a filled histogram on top of 
the fitted backgrounds, %both after the global fit (indicated as ``best fit") and 
as expected from the SM (indicated as $\mu=1.0$),
and, unstacked as an unfilled histogram, scaled by the factor indicated in the legend. 
The dashed histogram shows the total background as expected from the pre-fit 
MC simulation.
The size of the combined statistical and systematic uncertainty on the
sum of the signal and fitted background is indicated by the hatched band. The ratio
of the data to the sum of the signal and fitted background is shown in the lower panel.
\label{fig:App_BDTdistributions_1lepton}}
\end{figure}



\begin{figure}[tb!]
\begin{center}
\centerline{
\subfigure[$\ptv<120~\GeV$, 2 jets, 1-tag]{\includegraphics[width=0.3\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B0_J2_T1_L2_distMV1cBTag_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv>120~\GeV$, 2 jets, 1-tag]{\includegraphics[width=0.3\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B2_J2_T1_L2_distMV1cBTag_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv<120~\GeV$, 3 jets, 1-tag]{\includegraphics[width=0.3\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B0_J3_T1_L2_distMV1cBTag_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv>120~\GeV$, 3 jets, 1-tag]{\includegraphics[width=0.3\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B2_J3_T1_L2_distMV1cBTag_TType_GlobalFit_unconditionnal_mu1.pdf}}
}
%
\centerline{
\subfigure[$\ptv<120~\GeV$, 2 jets,  LL]{\includegraphics[width=0.3\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B0_J2_T2_L2_distmva_TTypell_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv>120~\GeV$, 2 jets, LL]{\includegraphics[width=0.3\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B2_J2_T2_L2_distmva_TTypell_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv<120~\GeV$, 3 jets, LL]{\includegraphics[width=0.3\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B0_J3_T2_L2_distmva_TTypell_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv>120~\GeV$, 3 jets, LL]{\includegraphics[width=0.3\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B2_J3_T2_L2_distmva_TTypell_GlobalFit_unconditionnal_mu1.pdf}}
}
%
\centerline{
\subfigure[$\ptv<120~\GeV$ 2 jets, MM+TT]{\includegraphics[width=0.3\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B0_J2_T2_L2_distmva_TTypexx_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv>120~\GeV$ 2 jets, MM+TT]{\includegraphics[width=0.3\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B2_J2_T2_L2_distmva_TTypexx_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv<120~\GeV$, 3 jets, MM+TT]{\includegraphics[width=0.3\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B0_J3_T2_L2_distmva_TTypexx_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[$\ptv>120~\GeV$, 3 jets, MM+TT]{\includegraphics[width=0.3\textwidth]{Figures/Appendix/BDTAllRegions/Region_Y2012_isMVA1_B2_J3_T2_L2_distmva_TTypexx_GlobalFit_unconditionnal_mu1.pdf}}
}
\caption{
The distributions input to the global MVA fit in the 2-lepton channel:
(a)--(d) MV1c-algorithm output distributions in the 1-tag control regions 
and
(e)--(l) BDT$_{VH}$-discriminant distributions in the 2-tag signal regions.
Shown are the data (points with error bars) and expectation (histograms).
The analysis regions (in terms of $\ptv$ range, jet multiplicity and $b$-tag region)
are indicated in the subfigure captions. 
The bin left boundaries in (a)--(d) denote 
the operating points ({\it{MV1c(b) OP}}) as defined in section~\ref{sec:reco},
corresponding to 
$b$-tagging efficiencies of 80\%, 70\%, 60\%, 50\%,
i.e., the $b$-jet purity increases from left to right.      
The background contributions after the global fit of the MVA are shown 
as filled histograms.
The Higgs boson signal ($\mh = 125$~GeV) is shown as a filled histogram on top of 
the fitted backgrounds, %both after the global fit (indicated as ``best fit") and 
as expected from the SM (indicated as $\mu=1.0$),
and, unstacked as an unfilled histogram, scaled by the factor indicated in the legend. 
The dashed histogram shows the total background as expected from the pre-fit 
MC simulation.
The size of the combined statistical and systematic uncertainty on the
sum of the signal and fitted background is indicated by the hatched band. The ratio
of the data to the sum of the signal and fitted background is shown in the lower panel.
\label{fig:App_BDTdistributions_2lepton}}
\end{center}
\end{figure}



==> App_Plots_Legend.tex <==

\begin{figure}[hbtp!]
\begin{center}
\includegraphics[width=0.4\textwidth]{Figures/Appendix/Legend/legend.pdf}
\caption{A large version of the legend.
\label{fig:App_Legend}}
\end{center}
\end{figure}
%






	
  


==> App_Plots_MVAinputs.tex <==



%
% Input Variables for 0-lepton in 2-jet, 2-tags (LL+MM+TT), hight ptV
% For now: put the full list, also the ones already shown in the main body of the paper (Fig. 1) 
% 
% 10 plots in total, arrange in 3 columns (4 rows)
% 
\begin{figure}[tb!]
% Row 1
  \vspace{-20pt}

\centerline{
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L0_distMET_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L0_distpTB1_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L0_distpTB2_TType_GlobalFit_unconditionnal_mu1.pdf}}
}
% Row 2
\centerline{
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L0_distmBB_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L0_distdRBB_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L0_distdEtaBB_TType_GlobalFit_unconditionnal_mu1.pdf}}
}
% Row 3
\centerline{
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L0_distdPhiVBB_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L0_distMEff_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L0_distMV1cB1_TType_GlobalFit_unconditionnal_mu1.pdf}}
}
% Row 4
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L0_distMV1cB2_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
  \vspace{-10pt}
\caption{
BDT input variables in the 0-lepton channel for the 2-jet 2-tag category (LL, MM and TT combined) and $\ptv > 120 \GeV$:
(a) \met, 
(b) $\pt(b_1)$,
(c) $\pt(b_2)$,
(d) \mbb, 
(e) $\Delta R(b_1,b_2)$,
(f) $|\Delta\eta(b_1,b_2)|$, 
(g) $\Delta\phi(V,bb)$,
%(h) $m_{\mathrm{Eff}}$,
(h) $H_{\mathrm{T}}$.
%(i) $MV1c(b_1)$~$OP$,
%(j) $MV1c(b_2)$~$OP$.
In (i) and (j) the output of the MV1c $b$-taging algorithm
is shown for the first and second identified $b$-jets, where the left bin 
boundaries denote the operating points ($MV1c(b_{1/2})$~$OP$)
of the MV1c $b$-tagging algorithm as defined in section~\ref{sec:reco},
corresponding to $b$-tagging efficiencies of 80\%, 70\%, 60\%, 50\%.
Background contributions after adjustments explained in the text are shown 
as filled histograms.
The Higgs boson signal ($\mh = 125$~GeV) is shown as a filled histogram on top of 
the fitted backgrounds, %both after the global fit (indicated as ``best fit'') and 
as expected from the SM (indicated as $\mu=1.0$),
and, unstacked as an unfilled histogram, scaled by the factor indicated in the legend. 
%and also separately as red histogram normalised to the same area as the total background. 
The dashed histogram shows the total background as expected from the pre-fit 
MC simulation. The entries in overflow are included in the last bin.
The combined statistical and systematic uncertainty on the
sum of the signal and fitted background is indicated by the hatched band. The ratio
of the data to the sum of the signal and fitted background is shown in the lower panel.
\label{fig:App_InputsMVA_0lepton}}
\end{figure}
%

%
% Input Variables for 1-lepton in 2-jet, 2-tags (LL+MM+TT), hight ptV
% For now: put the full list, also the ones already shown in the main body of the paper (Fig. 1) 
% 
% 11 plots in total, arrange in 3 columns (4 rows)
% 
\begin{figure}[tb!]
% Row 1
  \vspace{-20pt}
\centerline{
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L1_distpTV_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L1_distMET_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L1_distpTB1_TType_GlobalFit_unconditionnal_mu1.pdf}}
}
% Row 2
\centerline{
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L1_distpTB2_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L1_distmBB_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L1_distdRBB_TType_GlobalFit_unconditionnal_mu1.pdf}}
}
% Row 3
\centerline{
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L1_distdPhiVBB_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L1_distdPhiLBmin_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L1_distmTW_TType_GlobalFit_unconditionnal_mu1.pdf}}
}
% Row 4
\centerline{
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L1_distMV1cB1_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L1_distMV1cB2_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
}
  \vspace{-10pt}
\caption{
BDT input variables in the 1-lepton channel for the 2-jet 2-tag category (LL, MM and TT combined) and $\ptv > 120 \GeV$:
(a) \ptv,
(b) \met, 
(c) $\pt(b_1)$,
(d) $\pt(b_2)$,
(e) \mbb, 
(f) $\Delta R(b_1,b_2)$,
(g) $\Delta\phi(V,bb)$,
(h) $\mathrm{min}[\Delta\phi(\ell,b)]$,
(i) \mtw.
%(j) $MV1c(b_1)$~$OP$,
%(k) $MV1c(b_2)$~$OP$.
In (j) and (k) the output of the MV1c $b$-taging algorithm
is shown for the first and second identified $b$-jets, where the left bin 
boundaries denote the operating points ($MV1c(b_{1/2})$~$OP$)
of the MV1c $b$-tagging algorithm as defined in section~\ref{sec:reco},
corresponding to $b$-tagging efficiencies of 80\%, 70\%, 60\%, 50\%.
Background contributions after the adjustments explained in the text are shown 
as filled histograms.
The Higgs boson signal ($\mh = 125$~GeV) is shown as a filled histogram on top of 
the fitted backgrounds, %both after the global fit (indicated as ``best fit'') and 
as expected from the SM (indicated as $\mu=1.0$),
and, unstacked as an unfilled histogram, scaled by the factor indicated in the legend. 
%and also separately as red histogram normalised to the same area as the total background. 
The dashed histogram shows the total background as expected from the pre-fit 
MC simulation. The entries in overflow are included in the last bin.
The combined statistical and systematic uncertainty on the
sum of the signal and fitted background is indicated by the hatched band. The ratio
of the data to the sum of the signal and fitted background is shown in the lower panel.
\label{fig:App_InputsMVA_1lepton}}
\end{figure}
%

%
% Input Variables for 2-lepton in 2-jet, 2-tags (LL+MM+TT), hight ptV
% For now: put the full list, also the ones already shown in the main body of the paper (Fig. 1) 
% 
% 12 plots in total, arrange in 3 columns (4 rows)
% 
\begin{figure}[tb!]
% Row 1
  \vspace{-20pt}

\centerline{
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L2_distpTV_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L2_distMET_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L2_distpTB1_TType_GlobalFit_unconditionnal_mu1.pdf}}
}
% Row 2
\centerline{
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L2_distpTB2_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L2_distmBB_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L2_distdRBB_TType_GlobalFit_unconditionnal_mu1.pdf}}
}
% Row 3
\centerline{
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L2_distdEtaBB_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L2_distdPhiVBB_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L2_distdEtaVBB_TType_GlobalFit_unconditionnal_mu1.pdf}}
}
% Row 4
\centerline{
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L2_distmLL_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L2_distMV1cB1_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.25\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J2_T2_L2_distMV1cB2_TType_GlobalFit_unconditionnal_mu1.pdf}}
}
  \vspace{-10pt}
\caption{
BDT input variables in the 2-lepton channel for the 2-jet 2-tag category (LL, MM and TT combined) and $\ptv > 120 \GeV$:
(a) \ptv,
(b) \met, 
(c) $\pt(b_1)$,
(d) $\pt(b_2)$,
(e) \mbb, 
(f) $\Delta R(b_1,b_2)$,
(g) $|\Delta\eta(b_1,b_2)|$, 
(h) $\Delta\phi(V,bb)$,
(i) $|\Delta\eta(V,bb)|$
(j) \mll.
%(k) $MV1c(b_1)$~$OP$,
%(l) $MV1c(b_2)$~$OP$.
In (k) and (l) the output of the MV1c $b$-taging algorithm
is shown for the first and second identified $b$-jets, where the left bin 
boundaries denote the operating points ($MV1c(b_{1/2})$~$OP$) 
of the MV1c $b$-tagging algorithm as defined in section~\ref{sec:reco},
corresponding to $b$-tagging efficiencies of 80\%, 70\%, 60\%, 50\%.
The distributions are shown after having applied the kinematic fit
as described in section~\ref{sec:selec}.       
Background contributions after the adjustments explained in the text are shown 
as filled histograms.
The Higgs boson signal ($\mh = 125$~GeV) is shown as a filled histogram on top of 
the fitted backgrounds, %both after the global fit (indicated as ``best fit'') and 
as expected from the SM (indicated as $\mu=1.0$),
and, unstacked as an unfilled histogram, scaled by the factor indicated in the legend. 
%and also separately as red histogram normalised to the same area as the total background. 
The dashed histogram shows the total background as expected from the pre-fit 
MC simulation. The entries in overflow are included in the last bin.
The combined statistical and systematic uncertainty on the
sum of the signal and fitted background is indicated by the hatched band. The ratio
of the data to the sum of the signal and fitted background is shown in the lower panel.
\label{fig:App_InputsMVA_2lepton}}
\end{figure}
%


%
% 3-jet specific Input Variables for 0/1/2-lepton in 3-jet, 2-tags (LL+MM+TT), hight ptV
% 
% 6 plots in total, arrange in 2 columns (3 rows)
% 
\begin{figure}[tb!]
% Row 1
\centerline{
\hfill
\subfigure[]{\includegraphics[width=0.36\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J3_T2_L0_distpTJ3_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.36\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J3_T2_L0_distmBBJ_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
}
% Row 2
\centerline{
\hfill
\subfigure[]{\includegraphics[width=0.36\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J3_T2_L1_distpTJ3_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.36\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J3_T2_L1_distmBBJ_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
}
% Row 3
\centerline{
\hfill
\subfigure[]{\includegraphics[width=0.36\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J3_T2_L2_distpTJ3_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.36\textwidth]{Figures/Appendix/MVAInputs/Region_Y2012_isMVA1_B2_J3_T2_L2_distmBBJ_TType_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
}
\caption{
Variables input to the BDT specific for 3-jet events in 2-tag category (LL, MM and TT combined) and $\ptv > 120 \GeV$:
(a) 0-lepton, $\pt^{\mathrm{jet}_3}$; 
(b) 0-lepton, $m_{bbj}$;
(c) 1-lepton, $\pt^{\mathrm{jet}_3}$; 
(d) 1-lepton, $m_{bbj}$;
(e) 2-lepton, $\pt^{\mathrm{jet}_3}$; 
(f) 2-lepton, $m_{bbj}$.
The distributions for the 2-lepton channel in (e) and (f) are shown after having applied the kinematic fit
as described in section~\ref{sec:selec}.       
The background contributions after the adjustments explained in the text are shown 
as filled histograms.
The Higgs boson signal ($\mh = 125$~GeV) is shown as a filled histogram on top of 
the fitted backgrounds, %both after the global fit (indicated as ``best fit'') and 
as expected from the SM (indicated as $\mu=1.0$),
and, unstacked as an unfilled histogram, scaled by the factor indicated in the legend. 
%and also separately as red histogram normalised to the same area as the total background. 
The dashed histogram shows the total background as expected from the pre-fit 
MC simulation. The entries in overflow are included in the last bin.
The size of the combined statistical and systematic uncertainty on the
sum of the signal and fitted background is indicated by the hatched band. The ratio
of the data to the sum of the signal and fitted background is shown in the lower panel.
\label{fig:App_InputsMVA_3jets}}
\end{figure}
%







	
  


==> App_Plots_Results.tex <==

%
% The BG subtracted weighted mass plot separately for 0/1/2-leptons 
% 3 plots in 1 figure
%
\begin{figure}[tb!]
\begin{center}
\subfigure[]{\includegraphics[width=0.32\textwidth]{Figures/Appendix/Results/Region_L0_T2_B9_Y2012_distmjj_Higgsweighted_BkgSub_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.32\textwidth]{Figures/Appendix/Results/Region_L1_T2_B9_Y2012_distmjj_Higgsweighted_BkgSub_GlobalFit_unconditionnal_mu1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.32\textwidth]{Figures/Appendix/Results/Region_L2_T2_B9_Y2012_distmjj_Higgsweighted_BkgSub_GlobalFit_unconditionnal_mu1.pdf}}
\end{center}
\caption{The distribution of \mbb\ in data after subtraction of all backgrounds
except for the diboson processes 
%and for the associated $WH$ and $ZH$ production of a SM Higgs boson with $\mh=125$~GeV, 
as obtained with the dijet-mass analysis for the 8 TeV data for the 
(a) 0-lepton,
(b) 1-lepton, and
(c) 2-lepton channels.
The contributions from all
\ptv\ intervals, 
number-of-jets and 2-tag $b$-tagging categories are summed weighted by
their respective values of the ratio of expected Higgs boson signal to fitted background.
%The backgrounds are evaluated according to the results of the global fit.
The Higgs boson signal contribution is shown 
%both with its fitted signal strength (indicated as ``best fit") and 
as expected for the SM cross section (indicated as $\mu=1.0$).
The size of the combined statistical and systematic uncertainty
on the fitted background is indicated by the hatched band.
}
\label{fig:App_mbbBGsubtractedPerChannel}
\end{figure}


%
% The log(s/b) plot seprataely for 0/1/2-leptons
% 3 pllots in 1 figure
%
\begin{figure}[tb!]
\begin{center}
\subfigure[]{\includegraphics[width=0.32\textwidth]{Figures/Appendix/Results/Global_SoverB_2012_details_pulls_L0.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.32\textwidth]{Figures/Appendix/Results/Global_SoverB_2012_details_pulls_L1.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.32\textwidth]{Figures/Appendix/Results/Global_SoverB_2012_details_pulls_L2.pdf}}
\end{center}
\caption{Event yields as a function of $\log(S/B)$ for data, background
and Higgs boson signal with $\mh=125$~GeV for the 8~TeV dataset
%Update to combined
for the
(a) 0-lepton,
(b) 1-lepton
and
(c) 2-lepton
channels.
Final-discriminant bins in all signal regions 
are combined into bins of $\log(S/B)$
The signal $S$ and background $B$ yields are expected and fitted, respectively.
%and background yields $S$ and $B$ are evaluated according to the results of the global fit.{\bf (TBC)}
The Higgs boson signal contribution is shown 
%both with its fitted signal strength (indicated as ``best fit") and 
as expected for the SM cross section (indicated as $\mu=1.0$).
The pull of the data with respect to the background-only prediction is
also shown with statistical uncertainties only. 
The full line indicates the pull of the prediction for signal ($\mu=1.0$) and background
with respect to the background-only prediction.
}
\label{fig:App_logstob_individualChannels}
\end{figure}

\begin{figure}[tb!]
\begin{center}
\includegraphics[width=0.47\textwidth]{Figures/Appendix/Results/Global_SoverB_2012_details.pdf}
\end{center}
\caption{Event yields as a function of $\log(S/B)$ for data, background
and Higgs boson signal with $\mh=125$~GeV for the 8~TeV dataset.
%Update to combined
Final-discriminant bins in all signal regions 
are combined into bins of $\log(S/B)$.
The signal $S$ and background $B$ yields are expected and fitted, respectively.
%and background yields $S$ and $B$ are evaluated according to the results of the global fit.{\bf (TBC)}
The Higgs boson signal contribution is shown 
%both with its fitted signal strength (indicated as ``best fit") and 
as expected for the SM cross section (indicated as $\mu=1.0$).
The ratio of the data to the background-only prediction is also shown
with statistical uncertainties only. 
The full line indicates the ratio of the prediction for signal ($\mu=1.0$) and background
to the background-only prediction.
}
\label{fig:App_logstob_ratio}
\end{figure}









==> App_Plots_SevenTeVPtv.tex <==


%
% The 7 TeV ptv plots in the 2-tag signal regions
% 6 plots: arrange in 2 columns
\begin{figure}[tb!]
\begin{center}
\centerline{
\hfill
\subfigure[]{\includegraphics[width=0.36\textwidth]{Figures/Appendix/SevenTeVPtv/ZeroLepton_2T2J_B9_2011_VpT_GlobalFit_unconditionnal_mu1_logy.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.36\textwidth]{Figures/Appendix/SevenTeVPtv/ZeroLepton_2T3J_B9_2011_VpT_GlobalFit_unconditionnal_mu1_logy.pdf}}
\hfill
}
%
\centerline{
\hfill
\subfigure[]{\includegraphics[width=0.36\textwidth]{Figures/Appendix/SevenTeVPtv/OneLepton_2T2J_B9_2011_VpT_GlobalFit_unconditionnal_mu1_logy.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.36\textwidth]{Figures/Appendix/SevenTeVPtv/OneLepton_2T3J_B9_2011_VpT_GlobalFit_unconditionnal_mu1_logy.pdf}}
\hfill
}
%
\centerline{
\hfill
\subfigure[]{\includegraphics[width=0.36\textwidth]{Figures/Appendix/SevenTeVPtv/TwoLepton_2T2J_B9_2011_VpT_GlobalFit_unconditionnal_mu1_logy.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.36\textwidth]{Figures/Appendix/SevenTeVPtv/TwoLepton_2T3J_B9_2011_VpT_GlobalFit_unconditionnal_mu1_logy.pdf}}
\hfill
}
\end{center}
\caption{
The \ptv\ distributions observed in the 7~TeV data (points with error bars) and expected (histograms) 
for the 2-tag signal regions for
(a) 0-lepton, 2-jet;
(b) 0-lepton, 3-jet;
(c) 1-lepton, 2-jet;
(d) 1-lepton, 3-jet;
(e) 2-lepton, 2-jet;
(f) 2-lepton, 3-jet.
The background contributions after the global fit of the dijet-mass analysis are shown as filled histograms.
The Higgs boson signal ($\mh = 125$~GeV) is shown as a filled histogram on top of 
the fitted backgrounds, %both after the global fit (indicated as ``best fit") and 
as expected from the SM (indicated as $\mu=1.0$),
and, unstacked as an unfilled histogram, scaled by the factor indicated in the legend. 
The dashed histogram shows the total background as expected from the pre-fit 
MC simulation. The entries in overflow are included in the last bin.
The size of the combined statistical and systematic uncertainty on the
sum of the signal and fitted background is indicated by the hatched band. The ratio
of the data to the sum of the signal and fitted background is shown in the lower panel.
\label{fig:App_7Tev_ptv}}
\end{figure}


==> AuxiliaryMaterial.tex <==
\section{Auxiliary material}\label{auxiliarymaterial}

A large version of the legend is shown in figure~\ref{fig:App_Legend}.

\input{App_Plots_Legend.tex}

All input variables to the BDT for the
0-, 1- and 2-lepton channels are shown in 
figures~\ref{fig:App_InputsMVA_0lepton}--\ref{fig:App_InputsMVA_3jets}.
% figures~\ref{fig:App_InputsMVA_0lepton}, \ref{fig:App_InputsMVA_1lepton}, \ref{fig:App_InputsMVA_2lepton} and \ref{fig:App_InputsMVA_3jets}.

\input{App_Plots_MVAinputs.tex}

The \ptv\ distributions for the 2-tag signal regions
of the 7~TeV dijet-mass analysis are shown in figure~\ref{fig:App_7Tev_ptv}.

\input{App_Plots_SevenTeVPtv.tex}

All input distributions to the global MVA fit for the
0-, 1- and 2-lepton channels are shown in 
figures~\ref{fig:App_BDTdistributions_0lepton}--\ref{fig:App_BDTdistributions_2lepton}.
% figures~\ref{fig:App_BDTdistributions_0lepton}, \ref{fig:App_BDTdistributions_1lepton} and \ref{fig:App_BDTdistributions_2lepton}.

\input{App_Plots_BDTAllRegions.tex}

Additional material for the results section,
%splitting up results either for data taking periods (7 and 8~TeV) or 
split for the 8~TeV data in lepton-channels, 
is presented in figures~\ref{fig:App_mbbBGsubtractedPerChannel}--\ref{fig:App_logstob_ratio}. 
%and \ref{fig:App_logstob_individualChannels}.

\input{App_Plots_Results.tex}








	
  


==> Sec_SystTable1.tex <==

A similar approach is used to assess the contribution of groups of systematic uncertainties 
to the total systematic uncertainty on $\hat\mu$. All NPs associated with the uncertainties 
within a group are fixed to their fitted values and the fit is repeated. The difference in 
quadrature between the uncertainties on $\hat\mu$ from this fit and from the nominal fit 
provides an estimate of the systematic uncertainty attached to the considered group of uncertainties. 
A breakdown of systematic uncertainties obtained in this way for the MVA applied to the 8~TeV data 
is presented in table~\ref{tab:syst_unc}. 
Among the experimental systematic uncertainties, those related to jet properies (dominated by the
jet energy scale and resolution) and to $b$-tagging are the largest contributors to the total 
systematic uncertainty. Among the theoretical and modelling uncertainties, those on the signal 
and the $W$+jets background are the largest contributors, followed by those on the $Z$+jets and 
\ttb\ backgrounds.   



==> Sec_SystTable2.tex <==


\begin{table}[tb!]
\begin{center}
%\advance\leftskip -0.2cm
\begin{tabular}{ l | l  c | c }
\hline\hline
\multicolumn{2}{l}{Source of uncertainty} & $\sigma_\mu^+$ & $\sigma_\mu^-$ \\
\hline
\multicolumn{2}{l}{Total} & 0.43 & 0.40\\
\multicolumn{2}{l}{Statistical} & 0.33 & 0.32 \\
\multicolumn{2}{l}{Systematic} & 0.28 & 0.24 \\
\hline
\multicolumn{4}{l}{Experimental uncertainties}\\
\hline
\multicolumn{2}{l}{Jets} & 0.09 & 0.07 \\
\multicolumn{2}{l}{\met} & 0.03 & 0.02 \\
\multicolumn{2}{l}{Leptons} & 0.01 & 0.01 \\
\multirow{3}{*}{$b$-tagging$^{(\ast)}$~~~} & $b$-jets & 0.08 & 0.06 \\
& $c$-jets & 0.05 & 0.04 \\
& light jets & 0.04 & 0.04 \\
\multicolumn{2}{l}{Luminosity} & 0.04 & 0.02 \\
\hline
\multicolumn{4}{l}{Theoretical and modelling uncertainties}\\
\hline
\multicolumn{2}{l}{Signal} & 0.11 & 0.04 \\
\multicolumn{2}{l}{$W+$jets} & 0.12 & 0.12 \\
\multicolumn{2}{l}{$Z+$jets} & 0.08 & 0.08 \\ 
\multicolumn{2}{l}{\ttb} & 0.08 & 0.07 \\
\multicolumn{2}{l}{Single-top} & 0.05 & 0.04 \\
\multicolumn{2}{l}{Diboson} & 0.02 & 0.02 \\
\multicolumn{2}{l}{Multijet} & 0.06 & 0.06 \\
\hline\hline
\end{tabular}
\caption{Breakdown of the uncertainties on $\hat\mu$ obtained with the MVA applied to the 8~TeV data. 
The positive and negative uncertainties are denoted $\sigma_\mu^+$ and  $\sigma_\mu^-$, respectively. 
The individual sources of systematic uncertainty detailed in section~\ref{sec:sys} are combined into 
categories. The uncertainties on the background normalisations are included in the theoretical and 
modelling uncertainties. The sums in quadrature of the systematic uncertainties attached to the 
categories differ from the total systematic uncertainties due to correlations.
$(\ast)$ The positive and negative uncertainties due to $b$-tagging for all jet flavours combined 
are 0.11 and 0.09, respectively.
\label{tab:syst_unc}}
\end{center}
\end{table}


